Safe Reinforcement Learning with Scene Decomposition for Navigating Complex Urban Environments

Navigating urban environments represents a complex task for automated vehicles. They must reach their goal safely and efficiently while considering a multitude of traffic participants. We propose a modular decision making algorithm to autonomously navigate intersections, addressing challenges of existing rule-based and reinforcement learning (RL) approaches. We first present a safe RL algorithm relying on a model-checker to ensure safety guarantees. To make the decision strategy robust to perception errors and occlusions, we introduce a belief update technique using a learning based approach. Finally, we use a scene decomposition approach to scale our algorithm to environments with multiple traffic participants. We empirically demonstrate that our algorithm outperforms rule-based methods and reinforcement learning techniques on a complex intersection scenario.

==> scatterplot.tex <==
%auto-ignore
\begin{tikzpicture}[]
\begin{axis}[ylabel = {Collisions}, xlabel = {Steps}, grid=both, ymin = {0.0}, width=7cm]
\addplot+[draw=none, mark size = 4, mark=*, error bars/.cd, 
x dir=both, x explicit, y dir=both, y explicit]
table [
x error plus=ex+, x error minus=ex-, y error plus=ey+, y error minus=ey-
] {
x y ex+ ex- ey+ ey-
136.627 0.003 94.19082643 94.19082643 0.054717401 0.054717401
};
\addlegendentry{RL updater}
\addplot+[draw=none, mark size = 4, mark=*, error bars/.cd, 
x dir=both, x explicit, y dir=both, y explicit]
table [
x error plus=ex+, x error minus=ex-, y error plus=ey+, y error minus=ey-
] {
x y ex+ ex- ey+ ey-
365.301 0.001 81.06228156 81.06228156 0.031622777 0.031622777
};
\addlegendentry{baseline no updater}
\addplot+[draw=none, mark size = 4, mark=*, error bars/.cd, 
x dir=both, x explicit, y dir=both, y explicit]
table [
x error plus=ex+, x error minus=ex-, y error plus=ey+, y error minus=ey-
] {
x y ex+ ex- ey+ ey-
331.513 0.0 95.63173772 95.63173772 0.0 0.0
};
\addlegendentry{baseline updater}
\addplot+[draw=none, mark size = 4, mark=*, error bars/.cd, 
x dir=both, x explicit, y dir=both, y explicit]
table [
x error plus=ex+, x error minus=ex-, y error plus=ey+, y error minus=ey-
] {
x y ex+ ex- ey+ ey-
172.778 0.0 108.3850268 108.3850268 0.0 0.0
};
\addlegendentry{masked-RL updater}
\addplot+[
draw=none, mark size = 4, mark=*, error bars/.cd, 
x dir=both, x explicit, y dir=both, y explicit
]
table [
x error plus=ex+, x error minus=ex-, y error plus=ey+, y error minus=ey-
] {
x y ex+ ex- ey+ ey-
258.411 0.0 133.7956029 133.7956029 0.0 0.0
};
\addlegendentry{masked-baseline updater}
\end{axis}

\end{tikzpicture}


